Densest Subhypergraph: Negative Supermodular Functions and Strongly Localized Methods

Dense subgraph discovery is a fundamental primitive in graph and hypergraph analysis which among other applications has been used for real-time story detection on social media and improving access to data stores of social networking systems. We present several contributions for localized densest subgraph discovery, which seeks dense subgraphs located nearby given seed sets of nodes. We first introduce a generalization of a recent $\textit{anchored densest subgraph}$ problem, extending this previous objective to hypergraphs and also adding a tunable locality parameter that controls the extent to which the output set overlaps with seed nodes. Our primary technical contribution is to prove when it is possible to obtain a strongly-local algorithm for solving this problem, meaning that the runtime depends only on the size of the input set. We provide a strongly-local algorithm that applies whenever the locality parameter is not too small, and show via counterexample why strongly-local algorithms are impossible below a certain threshold. Along the way to proving our results for localized densest subgraph discovery, we also provide several advances in solving global dense subgraph discovery objectives. This includes the first strongly polynomial time algorithm for the densest supermodular set problem and a flow-based exact algorithm for a heavy and dense subgraph discovery problem in graphs with arbitrary node weights. We demonstrate our algorithms on several web-based data analysis tasks.

==> intro-david.tex <==
A common paradigm in in unsupervised data analysis is to take as input a graph or hypergraph and to output extremal subsets. The type of extremal subset range from sets of minimum cut to minimum sparsest cut to maximal clique~\cite{stuffhere}. The underlying hypothesis is that extremal set reflects a region of important and noteworthy structure with respect to the bulk properties of the graph that is \emph{informative} to a user — for exploratory data analysis — or useful downstream algorithm such as a graph partitioner or machine learning pipeline — for subset-based models. 

An issue with this paradigm is that the hypothesis may be trivially or unusefully true. For instance, the minimum cut set in an unweighted graph with any degree 1 node is just that single node, which yields little information; a set of minimum conductance may be a simple small subgraph that just happens to have a small number of bridge nodes back to the rest of the graph~\cite{leskovec2009}. A second and related challenge is that finding the extremal subset typically results in an NP-complete problem. Even if the problem is solved approximately, it may still consume substantial time. 

\emph{Localized} graph algorithms are a practical and efficient solution to this problem. The idea is that we rephrase the extremal search problem with respect to a reference set of nodes $R$. For instance, we may want the solution \emph{within} the set $R$ or \emph{nearby} the set $R$ with some measure of distance or fraction of $R$. This area has been most extensively developed in the space of algorithms for finding small conductance cuts in a graph where techniques range between spectral methods~\cite{andersen2006} and flow methods~\cite{lr2004,al2008,oz2013,veldt2019,liu2022}. These techniques have also been extended to hypergraph analysis~\cite{XXX}. For methods that are able to effectively \emph{grow} small subsets, then $R$ may be as small as a single node; whereas for other techniques that \emph{shrink or adapt} $R$, then $R$ must be considerably larger. Often, a goal with these algorithms is to get a strongly localized runtime guarantee such that the total runtime scales with the size of the output instead of the size of the input graph. Using a localized algorithm, then, enables one to analyze \emph{many} interesting sets in the graph by varying the reference set $R$. 

(NOTE, use whatever the standard term is… I can never reminder if it's densest subgraph/etc. because there are the two variations, the one Reid Andersen used in the SODA 2008 paper and the one that's computable in polytime.) 

As we previously mentioned, the space of localized graph algorithms has been most extensively explored in terms of sets with small \emph{cut} values. However, another perspective on extermal sets seeks \emph{high density} independently of cut values. The \emph{densest subgraph} is one such example that seeks a subgraph $S$ of maximum average degree. In a small surprise, this subset can be computed in polynomial time — either by a classic flow algorithm or a recent peeling algorithm that removes vertices from the graph one at a time to hone in on the densest subset. Localized algorithms are also possible for the densest subgraph problem as shown in~\cite{TheAnchoredDensestSubgraphPaper?} 

XXX-Make sure these are accurate…-XXX 

The contribution of our paper is to greatly expand the scope of possible algorithms for localized densest subgraph computations. First, we establish a parametric formulation of the discrete objective function underlying localized densest subgraph. This allows us to vary the degree of localization and continuously tradeoff between the degree of localization and the amoung of computation. We explicitly delinate the region of strong locality where the algorithms have a runtime that scales identify output size. Moreover, we show hypergraph generalizations of all of these algorithms. Our methods use max-flow / min-cut computations as a primative and we show counter-examples where standard \emph{peeling} methods cannot approximate these localized objective fucntions at all. Finally, we demonstrate the techniques on a variety of datasets.

==> intro-updated.tex <==
A common paradigm in unsupervised data analysis is to take as input a graph or hypergraph and to output extremal subsets. The types of extremal subsets range from sets of minimum cut~\cite{stoer1997simple} to minimum sparsest cut~\cite{matula1990sparsest} to maximal clique~\cite{bomze1999maximum}. The underlying hypothesis is that extremal sets reflect important and noteworthy structures that are informative for exploratory data analysis, or useful for downstream algorithms such as graph partitioners or machine learning pipelines that operate on subsets of the larger graph.
This basic paradigm is fundamental in Web analysis and applied to problems such as detecting real-time stories on social media~\cite{angel2014dense}, improving access to data stores of social-networking systems~\cite{gionis2013piggybacking}, and a wide variety of clustering and community detection tasks over web-based datasets~\cite{veldt2018correlation,leskovec2009community,andersen2006communities,flake2000efficient}.

An issue with this paradigm is that there are many cases where extremal sets are trivial or simply unuseful. For instance, the minimum cut set in an unweighted graph with any degree 1 node is just that single node, which yields little information; a set of minimum conductance may be a simple small subgraph that just happens to have a small number of bridges to the rest of the graph~\cite{leskovec2009community}. A second and related challenge is that finding the extremal subset typically results in an NP-complete problem. Even if solved approximately, it may still consume substantial time. 

\emph{Localized} graph algorithms are a practical solution to this problem. The idea is that we rephrase the extremal search problem with respect to a reference set of nodes $R$. For instance, we may want the solution \emph{within} $R$ or \emph{nearby} $R$ with some measure of distance or fraction of $R$. This area has been most \cutforspace{extensively}{} developed in the space of algorithms for finding small conductance cuts in a graph where techniques range between spectral methods~\cite{andersen2006communities,AndersenChungLang2006}, flow methods~\cite{LangRao2004,orecchia2014flow,Veldt2019flow,wang2017capacity,andersen2008algorithm,Fountoulakis2023flow}, and heat-kernel diffusions~\cite{kloster2014heat}. These techniques have also been extended to hypergraph analysis~\cite{VBKMinimizing2020,ibrahim2020local,liu2021strongly}. For methods that are able to effectively \emph{grow} small subsets, then $R$ may be as small as a single node; whereas for other techniques that \emph{shrink or adapt} $R$, then $R$ must be considerably larger. Often, a goal with these algorithms is to get a strongly localized runtime guarantee such that the total runtime scales with the size of the output instead of the size of the input graph. Using a localized algorithm enables one to analyze \emph{many} interesting sets in the graph by varying the reference set $R$. These localized algorithms have already been widely used in web-based data analysis tasks such as detecting related retail products on Amazon~\cite{kloster2014heat,Veldt2019flow,VBKHypergraph2020}, identifying groups of same-topic posts on Stackoverflow~\cite{VBKHypergraph2020}, clustering restaurants based on reviews on Yelp~\cite{liu2021strongly}, and finding communities in various types of online social networks~\cite{kloster2014heat,wang2017capacity,Veldt2019flow}.

Although many extremal set problems in graph analysis focus on finding small \emph{cut} values, another perspective on extremal sets seeks \emph{high density} independently of cut values. The \emph{densest subgraph} is one such example that seeks a subgraph $S$ of maximum average degree. In a small surprise, this subset can be computed in polynomial time by a classic flow algorithm~\cite{GolFinding1984} or via linear programming~\cite{ChaGreedy2000}. A simple peeling algorithm that removes vertices from the graph one at a time has long been known to be a 2-approximation for the problem~\cite{ChaGreedy2000}. More recently, an iterated peeling algorithm has been shown to converge to the optimal solution~\cite{CQTDensest2022}. Many variants and generalizations of the densest subgraph problem have been studied and considered (see~\cite{LMFBSurvey2023} for a very recent survey). One of the most general of these is the densest supermodular subset problem (DSS), where the goal is to maximize the ratio between a nonnegative monotone supermodular function $f$ and the size of the returned set. Localized variants of the densest subgraph problem have also been considered recently~\cite{DQCAnchored2022}. However, localized algorithms for dense subgraph discovery remain underexplored and remain far less understood than localized algorithms for finding small cuts.

In this paper we greatly expand the scope of possible algorithms for dense subgraph computations, both in terms of global and local variants of the problem. We first provide a simple reduction that leads to efficient exact algorithms for a more general version of the densest supermodular subset (DSS) problem where the supermodular function does not need to be nonnegative (Theorem~\ref{thm:general-to-nonnegative}). This captures several dense subgraph problems that are not special cases of the standard nonnegative DSS problem~\cite{MKFinding2018,DQCAnchored2022}. We then provide the first strongly polynomial algorithm for DSS (Algorithm~\ref{alg:density-improve}, Theorem~\ref{thm:strongly-polynomial}); previous approaches came with weakly polynomial runtimes. Our final contribution to \emph{global} dense subgraph discovery algorithms is to design a flow-based exact algorithm for finding the densest subset of a node-weighted graph or hypergraph. Prior research on this problem showed how to obtain efficient flow-based solutions in the case of graphs with strictly non-negative weights~\cite{GolFinding1984,FLD+Discovering2022}; our results show how this can be extended to arbitrary node weights (Section~\ref{sec:flow-based-exact}). 

In addition to our results for global dense subgraph discovery, we greatly advance the state of the art in localized densest subgraph computations (Section~\ref{sec:strongly-local-flow}). First, we establish a parametric formulation of the discrete objective function underlying localized densest subgraph discovery (Problems~\ref{prob:adsh},~\ref{prob:adshf}). This allows us to vary the degree of localization and continuously tradeoff between the degree of localization and the amount of computation. We explicitly delineate the region of strong locality where algorithms can have a runtime that scales independently of graph size (Theorem~\ref{thm:slocal}). Moreover, we show hypergraph generalizations of all of these algorithms. Our methods use max-flow / min-cut computations as a primitive and we show (in the appendix) counter-examples where standard \emph{peeling} methods cannot approximate these objectives  at all. 

We demonstrate the advantages of the techniques on a variety of web-relevant datasets. This includes a hypergraph of web domains where hypergraphs are induced by hosts (Section~\ref{sec:domain-hypergraph}). We show how our localized algorithms can help identify a densely connected set of about 1300 academic domains around the world. 
